Revisiting Meta-evaluation for Grammatical Error Correction

Metrics are the foundation for automatic evaluation in grammatical error correction (GEC), with their evaluation of the metrics (meta-evaluation) relying on their correlation with human judgments. However, conventional meta-evaluations in English GEC encounter several challenges including biases caused by inconsistencies in evaluation granularity, and an outdated setup using classical systems. These problems can lead to misinterpretation of metrics and potentially hinder the applicability of GEC techniques. To address these issues, this paper proposes SEEDA, a new dataset for GEC meta-evaluation. SEEDA consists of corrections with human ratings along two different granularities: edit-based and sentence-based, covering 12 state-of-the-art systems including large language models (LLMs), and two human corrections with different focuses. The results of improved correlations by aligning the granularity in the sentence-level meta-evaluation, suggest that edit-based metrics may have been underestimated in existing studies. Furthermore, correlations of most metrics decrease when changing from classical to neural systems, indicating that traditional metrics are relatively poor at evaluating fluently corrected sentences with many edits.

==> tables/tab_EBM_example.tex <==
% 表：編集ベース人手評価の流れ
\begin{table*}[t]
\centering
\begin{tabular*}{16cm}{l|ll}
\Hline
\multirow{2}{*}{\textbf{Step 1}} & \textbf{Source:} There is a story of a girl who \textcolor[rgb]{0.7,0.7,0.0}{lives} in \textcolor[rgb]{0.7,0.7,0.0}{\_} social media world every night \textcolor[rgb]{0.7,0.7,0.0}{in} eight years. \\
& \textbf{Output:} There is a story of a girl who \textcolor{red}{\textbf{[lives → alive]}} in \textcolor[rgb]{0.1,0.7,0.3}{\textbf{[ → the]}} social media world \\&every night \textcolor[rgb]{0.1,0.7,0.3}{\textbf{[in → for]}} eight years. \\
\hline
\textbf{Step 2} & \textbf{Source:} There is a story of a girl who \textcolor{red}{\textbf{[lives]}} in \textcolor[rgb]{0.1,0.7,0.3}{\textbf{[\_]}} social media world every night \textcolor[rgb]{0.1,0.7,0.3}{\textbf{[in]}} eight \\&years. \\
\hline
\textbf{Score} & $F_{0.5}$ \textrm{= 0.67, Precision = 0.67, Recall = 0.67} \\
\Hline
\end{tabular*}
\caption{An example of the edit-based evaluation process. In Step 1, errors in the source are represented in yellow, valid edits in green, and invalid edits in red. In Step 2, corrected errors are shown in green, while those not corrected are in red.}
\label{tab:edit-based flow}
\end{table*}
